On the instability of embeddings for recommender systems: the case of Matrix Factorization

Most state-of-the-art top-N collaborative recommender systems work by learning embeddings to jointly represent users and items. Learned embeddings are considered to be effective to solve a variety of tasks. Among others, providing and explaining recommendations. In this paper we question the reliability of the embeddings learned by Matrix Factorization (MF). We empirically demonstrate that, by simply changing the initial values assigned to the latent factors, the same MF method generates very different embeddings of items and users, and we highlight that this effect is stronger for less popular items. To overcome these drawbacks, we present a generalization of MF, called Nearest Neighbors Matrix Factorization (NNMF). The new method propagates the information about items and users to their neighbors, speeding up the training procedure and extending the amount of information that supports recommendations and representations. We describe the NNMF variants of three common MF approaches, and with extensive experiments on five different datasets we show that they strongly mitigate the instability issues of the original MF versions and they improve the accuracy of recommendations on the long-tail.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.


==> original-intro.tex <==
\section{Introduction}
\label{sec:introduction}

Most state-of-the-art Top-N collaborative recommender systems work by learning embeddings to jointly represent users and items \cite{puresvd, he2017neural, xue2017deep}. 
Embeddings are derived in such a way that similar items (or similar users) have similar embeddings \cite{liang2016factorization}.
Embeddings can be learnt with either Matrix Factorization (MF) or deep learning (DL) techniques \cite{koren2009matrix, he2017neural}.
For both families of techniques, the learning procedure requires to sample the interaction space during the training (e.g., stochastic-gradient-descent \cite{ruder2016overview}, skip-grams with negative sampling \cite{mikolov2013linguistic}).

Embedding-based models are characterized by various sources of randomness in their training, such as the initial values of the embeddings and the sampled interactions.
Different random seeds or random generators might lead to different results, both in terms of embeddings learnt and items recommended.
If these differences are within a tolerance range, we can consider the algorithm to be stable in its recommendations.
However, if these differences are too large (i.e, if the algorithm is not stable), we cannot consider the recommendations to be reliable anymore, as the same algorithm executed on the same dataset could make totally different predictions for the same user-item pair \cite{madhyastha2019model}.

Note that our notion of stability of a recommender system is different from what has been commonly addressed in the literature. 
Some works focus on the stability of the model when you introduce noisy or malicious perturbations in the dataset \cite{said2012users}\cite{mobasher2007attacks}, or when the dataset evolves naturally with more interactions \cite{adomavicius2014improving}\cite{adomavicius2012stability}.
In this work we focus on the stability of the recommender system when the same model is trained on the same dataset in exactly the same experimental conditions but with a different random sequence (e.g., because of a different random seed).
Our definition of stability is strictly connected to that of \emph{repeatability} as defined, for instance, in the SIGIR Initiative to implement the ACM Artifact Review and Badging guidelines\footnote{\url{https://www.acm.org/publications/policies/artifact-review-badging}\\
According to this definition, an unstable algorithm is not repeatable}.

The variance in both the internal representation of the model (embeddings) and the output of the model (estimated relevance) can be reduced if enough samples are collected for each user and item to be modeled.
Unfortunately, most datasets exhibit strong popularity biases \cite{anderson2006long}. 
For instance, in the Netflix dataset, 1\% of the items account for 20\% of the interactions \cite{puresvd}.
Because of this biases, unpopular items (i.e., items with very few interactions) and short-profile users (i.e., users with very few interactions) will not collect enough samples during their training to smooth out the noise introduced by the randomness.
Embeddings learnt on a small sample size will be biased and unstable \cite{skurichina1998bagging}. 
As such, we expect the embeddings of unpopular items and short-profile users to vary greatly across different runs of the same experiment.

Different techniques exist to improve the generalization capabilities of a model by leveraging or controlling the randomness of the training procedure.
Bagging (i.e., bootstrapping and aggregating) is an ensemble method commonly used for classification problems \cite{skurichina1998bagging}. 
Bagging trains different models from boostrap replica of the same dataset and average their predictions. 
Bagging requires to retrain the same model several times: typically, more than 25 replicas are required in order to have an average model with a quality better than that of one single model \cite{skurichina1998bagging}. 
Moreover, bagging is designed to improve the generalization capabilities and not to stabilize the model \cite{skurichina1998bagging}.
Embeddings learnt on very small sample sizes have bad expected quality and large instability. 
In this case, bagging, which tries to improve the original training set, cannot help and can even increase the generalization error.
Other techniques, such as Stochastic Weight Averaging (SWA), produce an ensemble by averaging the weights of the same model at different epochs of the training process \cite{madhyastha2019model}\cite{izmailov2018averaging}.
In case of linear models, such as with Matrix Factorization, this is equivalent to averaging the embedding vectors during the gradient descent optimization. 
%The esembling is performed across different snaphshots of the same embedding during the training.
%ensembles in the model space
%combine several models and then use models’ predictions to produce the final prediction.
% ensembling in the weights space. 
%This method produces an ensemble by combining weights of the same network at different stages of training 
All these techniques are model agnostic and do not take into account the neighborhood properties of user and item embeddings: similar items (users) have similar embeddings.
In this work we propose a different averaging technique, in which items (users) embeddings are learnt as a weighted average of the embeddings of similar items (users). 

In this paper, we focus on the stability of Matrix Factorization models as a function of random-seed. 
We are especially interested in investigating if Matrix Factorization based models under different initializations of latent factors generated by distinct random seeds, produce similar predictions and similar embeddings.
%Collaborative Filtering (CF) approaches are known to be strongly biased towards the recommendation of popular items.
%While the recommendation of popular items is trivial, correctly guessing items that belong to the long-tail, a term forged by Anderson in \cite{anderson2006long}, is a challenging task that allows to improve the novelty of the recommendations provided by a Recommender System \gabbo{Attenzione, questa è una assunzione un po' forte}.
%The importance of enhancing novelty and diversity of the items in the recommendation lists has been widely discussed in the literature, and it has been shown that more diverse recommendations improve the quality of user's experience with the system\cite{kunaver2017diversity}.

%Matrix factorization (MF) methods are one of the most successful instances of CF\cite{koren2009matrix}. 
%Since the Netflix prize until today, those methods have been inspiring the research community and have been successfully employed in commercial applications.
%In its basic form, MF consists in representing users and items in a common latent factor space of a given dimension, while interactions are modeled by the dot product of user-item representations in that space\cite{ricci2011introduction}.

%Among CF techniques, MF is known to be less biased towards popularity with respect to many other collaborative approaches\cite{abdollahpouri2019unfairness, channamsetty2017recommender, whatrecommendersrecommend}.
%However, a doubt about the real quality of MF models recommendations on the long-tail raises from a simple consideration over the data used in their training procedures.
%During the training phase, the available data is represented by positive interactions given by users to items. 
%But the missing ones, which are the vast majority, are not considered at all, except for some particular optimization procedures, like BPR\cite{BPR}, where only a very small part is assumed as negative.
%In this paper we investigate the consequencies of that dependency under different aspects.
%We discuss which are the problems that such a dependency might induce, from the accuracy on the long-tail, to the stability of recommendations and latent representations in the new space.

We propose a new framework called Nearest Neighbors Matrix Factorization (NNMF), a generalization of classic Matrix Factorization that merges MF with nearest neighbors (NN) in order to alleviate the effects brought by the scarcity of interactions for unpopular items.
While in classic MF the latent representations of items or users are treated independently, in NNMF we force each embedding to be a linear combination of the embeddings of a set of their most similar neighbors.
With this approach we map the neighborhood relationships among items or users from the original interaction space to the new latent space.
This mapping has the effect to propagate the updates applied to an item or a user also to their respective neighbors.
Thanks to this property, less popular (i.e., less sampled) items or users get updated more often, e.g., whenever a neighbor item or user is updated.

We provide an extensive set of experiments, testing NNMF with three MF approaches (\bprmf, \funkmf and \pmf) over five different datasets. 
The results show that: 
\begin{itemize}
\item 
all the three MF methods suffer from the instability problem:
on average, recommended items change by more than 50\% by simply retraining the same model with a different random seed;
%and that are not always more accurate on the long-tail with respect to common collaborative baselines.
\item 
the three NNMF variants greatly improve stability: changing the random seed impacts the recommended items by less than 25\%;
\item 
the NNMF variants have better accuracy with respect to the original MF methods, as well as other baselines, in almost all measures and datasets;
\item
the improved stability and the information propagation of NNMF allow to reach convergence in a fraction of the number of epochs required by MF. 
\end{itemize}

The rest of the paper is organized as follows.
In Section \ref{sec:related-works} we list a set of works related to the argument we treat in this paper.
In Section \ref{sec:models} we introduce the issues of classic Matrix Factorization techniques and we present our new framework called Nearest Neighbor Matrix Factorization. We also describe some practical implementations over three well known MF algorithms.
In Section \ref{sec:experiments} we discuss the results obtained by an extensive set of experiments over a variety of different datasets, testing the performance of the new models under different aspects.
Finally, in Section \ref{sec:conclusions}, we provide some concluding remarks.

\section{Related Work}
\label{sec:related-works}

There exists different definitions of stability of a recommender system in the literature, and different ways to improve each of these definitions.
Most works define the stability of recommender system as the "consistent agreement of predictions" made to the same user by the same algorithm, when new incoming interactions  are added to the system in complete agreement to system’s prior predictions \cite{adomavicius2012stability}. 
For instance, the work in \cite{adomavicius2014improving} adopts bagging and iterative smoothing in conjunction with different traditional recommendation algorithms to improve their consistency. 
Other works define stability as the ability of the recommender system to provide consistent recommendations when malicious perturbations are performed to the dataset \cite{adomavicius2012stability}.
The work in \cite{mobasher2007attacks} suggests hybrid collaborative and content-based filtering as the best solution to mitigate the effects of attacks on the consistency of recommendations. 
Finally, other works \cite{said2018coherence} relate the stability, or confidence, of a recommender system with the quality of a dataset, either at system level (the magic barrier described in \cite{said2018coherence}) or at user-level \cite{dacrema2018eigenvalue}.
Our definition of stability -- the consistency of both recommendations and latent representations of users and items when the same model is trained on exactly the same dataset with a different random sequence -- is different from the definitions used in the literature. 

There are also several works in the literature that try to control (or leverage) the randomness intrinsic in machine learning algorithms in order to improve the generalization capabilities of a model.
Bagging is the most widely adopted black-box method used to leverage randomness in the input data in order improve the classification accuracy of a model \cite{skurichina1998bagging}. 
Bagging builds an ensemble of models by (i) running the same training algorithm on different boostrap replica of the same dataset and (ii) by aggregating their predictions. 
Training multiple model for prediction averaging, as with bagging, is computationally expensive. 
Therefore, other works train a single model and save the model parameters (snapshots) along the optimization path. 
The predictions of the snapshot models are later combined to produce the final prediction \cite{huang2017snapshot}.
Differently from bagging and snapshots, that build ensambles in the model space, other works build ensembles in the weights space. 
For instance, the works in \cite{madhyastha2019model} and \cite{izmailov2018averaging} use two variants of the same technique, Stochastic Weight Averaging (SWA), to compute a running average of the model weights during the last epochs of the training process.

